Finite-Width Neural Tangent Kernels from Feynman Diagrams

Neural tangent kernels (NTKs) are a powerful tool for analyzing deep, non-linear neural networks. In the infinite-width limit, NTKs can easily be computed for most common architectures, yielding full analytic control over the training dynamics. However, at infinite width, important properties of training such as NTK evolution or feature learning are absent. Nevertheless, finite width effects can be included by computing corrections to the Gaussian statistics at infinite width. We introduce Feynman diagrams for computing finite-width corrections to NTK statistics. These dramatically simplify the necessary algebraic manipulations and enable the computation of layer-wise recursion relations for arbitrary statistics involving preactivations, NTKs and certain higher-derivative tensors (dNTK and ddNTK) required to predict the training dynamics at leading order. We demonstrate the feasibility of our framework by extending stability results for deep networks from preactivations to NTKs and proving the absence of finite-width corrections for scale-invariant nonlinearities such as ReLU on the diagonal of the Gram matrix of the NTK. We numerically implement the complete set of equations necessary to compute the first-order corrections for arbitrary inputs and demonstrate that the results follow the statistics of sampled neural networks for widths $n\gtrsim 20$.

==> icml_2026_content/feynman_setup.tex <==
\RequirePackage{tikz}
\usetikzlibrary{shapes, arrows, positioning, decorations, fadings, external}
%\tikzexternalize[prefix=tikz/]
%\tikzsetfigurename{output-figure}
%the two lines above activate externalization!

\RequirePackage{tikz-feynman}
\RequirePackage{feynmp-auto}

\pgfdeclaredecoration{parallel}{initial}{%
  \state{initial}[width=0, next state=main]{\pgfpathmoveto{\pgfpointorigin}}%
  \state{main}[width=\pgfdecoratedinputsegmentlength/100]
  {
    \pgfpathlineto{\pgfpointorigin}
  }%
  \state{final}{}%
}

\tikzfeynmanset{
    color6color1ddntknew/.style={
    dash pattern=on 1pt off 1pt,
    line width=1pt,
    draw=color6,
    opacity=0,
    postaction={
        draw=color1,
        opacity=1,
        decorate,
        decoration={parallel, raise=-0.75pt}
        },
    postaction={
        draw=color6,
        opacity=1,
        decorate,
        decoration={parallel, raise=0.75pt}
        }
    },
    color6color1ddntk2new/.style={
    dash pattern=on 1pt off 1pt,
    line width=1pt,
    draw=color6,
    opacity=0,
    postaction={
        draw=color6,
        opacity=1,
        decorate,
        decoration={parallel, raise=-0.75pt}
        },
    postaction={
        draw=color1,
        opacity=1,
        decorate,
        decoration={parallel, raise=0.75pt}
        }
    },
    color6color2ddntknew/.style={
    dash pattern=on 1pt off 1pt,
    line width=1pt,
    draw=color6,
    opacity=0,
    postaction={
        draw=color2,
        opacity=1,
        decorate,
        decoration={parallel, raise=-0.75pt}
        },
    postaction={
        draw=color6,
        opacity=1,
        decorate,
        decoration={parallel, raise=0.75pt}
        }
    },
    color6color2ddntk2new/.style={
    dash pattern=on 1pt off 1pt,
    line width=1pt,
    draw=color6,
    opacity=0,
    postaction={
        draw=color6,
        opacity=1,
        decorate,
        decoration={parallel, raise=-0.75pt}
        },
    postaction={
        draw=color2,
        opacity=1,
        decorate,
        decoration={parallel, raise=0.75pt}
        }
    },
    color6color1color2ddntknew/.style={
    dash pattern=on 1pt off 1pt,
    line width=1pt,
    draw=color1,
    postaction={
        draw=color2,
        decorate,
        decoration={parallel, raise=-1.5pt}
        },
    postaction={
        draw=color6,
        decorate,
        decoration={parallel, raise=1.5pt}
        },
    },
    quarticblob/.style={
        /tikz/shape=circle,
        /tikz/draw=black,
        /tikz/fill=white!70!black,
        % tikzfeynman/particle={},
        /tikz/graphs/as={},
        /tikz/minimum size=15pt,
        % node contents={},
    },
    smallblob/.style={
        /tikz/shape=circle,
        /tikz/draw=black,
        /tikz/fill=white!70!black,
        % tikzfeynman/particle={},
        /tikz/graphs/as={},
        /tikz/minimum size=6pt,
        /tikz/inner sep=0pt,
        % node contents={},
    },
    propblob/.style={
      /tikz/shape=circle,
      /tikz/draw=black,
      /tikz/fill=white,
      % tikzfeynman/particle={},
      /tikz/graphs/as={},
      /tikz/minimum size=15pt,
      % node contents={},
    },
    color6color1color2ddntk2new/.style={
    dash pattern=on 1pt off 1pt,
    line width=1pt,
    draw=color1,
    postaction={
        draw=color6,
        decorate,
        decoration={parallel, raise=-1.5pt}
        },
    postaction={
        draw=color2,
        decorate,
        decoration={parallel, raise=1.5pt}
        },
    },
    minidot/.style={
        /tikz/shape=circle,
        /tikz/draw=black,
        /tikz/fill=black,
        /tikz/graphs/as={},
        /tikz/inner sep=0pt,
        /tikz/outer sep=0pt,
        /tikz/minimum size=0.75mm,
    },
    meddot/.style={
        /tikz/shape=circle,
        /tikz/draw=black,
        /tikz/fill=gray,
        /tikz/graphs/as={},
        /tikz/inner sep=0pt,
        /tikz/outer sep=0pt,
        /tikz/minimum size=5mm,
    },
    color1doubghost/.style={
    transform canvas={shift={(0,-1pt)}},
    dash pattern=on 3pt off 3pt,
    line width=1pt,
    draw=color1,
    preaction={
      transform canvas={shift={(0,1pt)}},
      dash pattern=on 3pt off 3pt,
      line width=1pt,
      draw=color1
     }
    },
    color2doubghost/.style={
    transform canvas={shift={(0,-1pt)}},
    dash pattern=on 3pt off 3pt,
    line width=1pt,
    draw=color2,
    preaction={
      transform canvas={shift={(0,1pt)}},
      dash pattern=on 3pt off 3pt,
      line width=1pt,
      draw=color2
     }
    },
    doubghost/.style={
        dashed,
        double distance=1.5pt,
        thick,
    },
    color1blackghost/.style={
    transform canvas={shift={(0pt,-1pt)}},
    line width=1pt,
    preaction={
      transform canvas={shift={(0pt,1pt)}},
      dash pattern=on 3pt off 3pt,
      line width=1pt,
      draw=color1
    }
    },
    blackcolor1ghost/.style={
    transform canvas={shift={(0pt,-1pt)}},
    dash pattern=on 3pt off 3pt,
    line width=1pt,
    draw=color1,
    preaction={
      transform canvas={shift={(0pt,1pt)}},
      line width=1pt,
      draw=black
    }
    },
    color2blackghost/.style={
    transform canvas={shift={(0pt,-1pt)}},
    line width=1pt,
    preaction={
      transform canvas={shift={(0pt,1pt)}},
      dash pattern=on 3pt off 3pt,
      line width=1pt,
      draw=color2
    }
    },
    blackcolor2ghost/.style={
    transform canvas={shift={(0pt,-1pt)}},
    dash pattern=on 3pt off 3pt,
    line width=1pt,
    draw=color2,
    preaction={
      transform canvas={shift={(0pt,1pt)}},
      line width=1pt,
      draw=black
    }
    },
    color1color2dntknew/.style={
    dash pattern=on 1pt off 1pt,
    line width=1pt,
    draw=color6,
    opacity=0,
    postaction={
        draw=color1,
        opacity=1,
        decorate,
        decoration={parallel, raise=-0.75pt}
        },
    postaction={
        draw=color2,
        opacity=1,
        decorate,
        decoration={parallel, raise=0.75pt}
        }
    },
    color2color1dntknew/.style={
    dash pattern=on 1pt off 1pt,
    line width=1pt,
    draw=color6,
    opacity=0,
    postaction={
        draw=color2,
        opacity=1,
        decorate,
        decoration={parallel, raise=-0.75pt}
        },
    postaction={
        draw=color1,
        opacity=1,
        decorate,
        decoration={parallel, raise=0.75pt}
        }
    },
    color1color2blackghost/.style={
    transform canvas={shift={(0pt,-1pt)}},
    line width=1pt,
    draw=black,  
    preaction={
      transform canvas={shift={(0pt,1pt)}},
      dash pattern=on 3pt off 3pt,
      line width=1pt,
      draw=color2
      },
    preaction={
      transform canvas={shift={(0pt,2.5pt)}},
      dash pattern=on 3pt off 3pt,
      line width=1pt,
      draw=color1
      }  
    },
    blackcolor1color2ghost/.style={
    transform canvas={shift={(0pt,1pt)}},
    line width=1pt,
    draw=black,  
    preaction={
      transform canvas={shift={(0pt,-1pt)}},
      dash pattern=on 3pt off 3pt,
      line width=1pt,
      draw=color1
      },
    preaction={
      transform canvas={shift={(0pt,-2.5pt)}},
      dash pattern=on 3pt off 3pt,
      line width=1pt,
      draw=color2
      }  
    },
    ntkdntkcolor1color2/.style={
    transform canvas={shift={(0pt,1pt)}},
    dash pattern=on 3pt off 3pt,
    line width=1pt,
    draw=color1,
    preaction={
      transform canvas={shift={(0pt,-1pt)}},
      dash pattern=on 3pt off 3pt,
      line width=1pt,
      draw=color1
      },
    preaction={
      transform canvas={shift={(0pt,-2.5pt)}},
      dash pattern=on 3pt off 3pt,
      line width=1pt,
      draw=color2
      }  
    },
    color1color2ghost/.style={
    transform canvas={shift={(0,-1pt)}},
    dash pattern=on 3pt off 3pt,
    line width=1pt,
    draw=color2,
    preaction={
      transform canvas={shift={(0,1pt)}},
      dash pattern=on 3pt off 3pt,
      line width=1pt,
      draw=color1
     }
    },
    color2color1ghost/.style={
    transform canvas={shift={(0,-1pt)}},
    dash pattern=on 3pt off 3pt,
    line width=1pt,
    draw=color1,
    preaction={
      transform canvas={shift={(0,1pt)}},
      dash pattern=on 3pt off 3pt,
      line width=1pt,
      draw=color2
    }
    },
    color6color6color1color2ghost/.style={
    transform canvas={shift={(0pt,1pt)}},
    dash pattern =on 3pt off 3pt,
    line width=1pt,
    draw=color6,
    preaction={
      transform canvas={shift={(0pt,-1pt)}},
      dash pattern=on 3pt off 3pt,
      line width=1pt,
      draw=color6
      },
    preaction={
      transform canvas={shift={(0pt,-2.5pt)}},
      dash pattern=on 3pt off 3pt,
      line width=1pt,
      draw=color1
      },
    preaction={
      transform canvas={shift={(0pt,-4pt)}},
      dash pattern=on 3pt off 3pt,
      line width=1pt,
      draw=color2
      }
    },
    color6color1color2ddntk/.style={
    dash pattern=on 0.5pt off 1pt,
    line width=1pt,
    draw=color6,
    preaction={
      transform canvas={shift={(1pt,-1.5pt)}},
      dash pattern=on 0.5pt off 1pt,
      line width=1pt,
      draw=color1
     },
    preaction={
      transform canvas={shift={(2pt,-3pt)}},
      dash pattern=on 0.5pt off 1pt,
      line width=1pt,
      draw=color2
      }  
    },
    color6color1ddntk/.style={
    dash pattern=on 0.5pt off 1pt,
    line width=1pt,
    draw=color6,
      preaction={
      transform canvas={shift={(1pt,2pt)}},
      dash pattern=on 0.5pt off 1pt,
      line width=1pt,
      draw=color1
      }  
    },    
    color6color2ddntk/.style={
    dash pattern=on 0.5pt off 1pt,
    line width=1pt,
    draw=color6,
      preaction={
      transform canvas={shift={(1pt,-1.5pt)}},
      dash pattern=on 0.5pt off 1pt,
      line width=1pt,
      draw=color2
      }  
    },
    color6color1ddntk2/.style={
    dash pattern=on 0.5pt off 1pt,
    line width=1pt,
    draw=color1,
      preaction={
      transform canvas={shift={(0pt,2.5pt)}},
      dash pattern=on 0.5pt off 1pt,
      line width=1pt,
      draw=color6
      }  
    },
    color6color2ddntk2/.style={
    dash pattern=on 0.5pt off 1pt,
    line width=1pt,
    draw=color2,
      preaction={
      transform canvas={shift={(1pt,-1.5pt)}},
      dash pattern=on 0.5pt off 1pt,
      line width=1pt,
      draw=color6
      }  
    },
    ddntkddntkcolor1color2ghost/.style={
    transform canvas={shift={(0pt,1.5pt)}},
    dash pattern=on 3pt off 3pt,
    line width=1pt,
    draw=color6,
    preaction={
      transform canvas={shift={(0pt,3pt)}},
      dash pattern=on 3pt off 3pt,
      line width=1pt,
      draw=color1
      },
    preaction={
      transform canvas={shift={(0pt,-1.5pt)}},
      dash pattern=on 3pt off 3pt,
      line width=1pt,
      draw=color6
      },
    preaction={
      transform canvas={shift={(0pt,-3pt)}},
      dash pattern=on 3pt off 3pt,
      line width=1pt,
      draw=color2
      }  
    },
    color6blackghost/.style={
    transform canvas={shift={(0pt,-1pt)}},
    line width=1pt,
    preaction={
      transform canvas={shift={(0pt,1pt)}},
      dash pattern=on 3pt off 3pt,
      line width=1pt,
      draw=color6
    }
    },
    blackcolor6ghost/.style={
    transform canvas={shift={(0pt,-1pt)}},
    dash pattern=on 3pt off 3pt,
    line width=1pt,
    draw=color6,
    preaction={
      transform canvas={shift={(0pt,1pt)}},
      line width=1pt,
      draw=black
    }
    },
    ntkdntkcolor2color2color6/.style={
    transform canvas={shift={(0pt,1pt)}},
    dash pattern=on 3pt off 3pt,
    line width=1pt,
    draw=color2,
    preaction={
      transform canvas={shift={(0pt,-1pt)}},
      dash pattern=on 3pt off 3pt,
      line width=1pt,
      draw=color2
      },
    preaction={
      transform canvas={shift={(0pt,-2.5pt)}},
      dash pattern=on 3pt off 3pt,
      line width=1pt,
      draw=color6
      }  
    },
    ntkdntkcolor6color1color1/.style={
    transform canvas={shift={(0pt,2.5pt)}},
    dash pattern=on 3pt off 3pt,
    line width=1pt,
    draw=color6,
    preaction={
      transform canvas={shift={(0pt,1pt)}},
      dash pattern=on 3pt off 3pt,
      line width=1pt,
      draw=color1
      },
    preaction={
      transform canvas={shift={(0pt,-1pt)}},
      dash pattern=on 3pt off 3pt,
      line width=1pt,
      draw=color1
      }  
    },
    ntkdntkcolor1color2color6/.style={
    transform canvas={shift={(0pt,1pt)}},
    dash pattern=on 3pt off 3pt,
    line width=1pt,
    draw=color1,
    preaction={
      transform canvas={shift={(0pt,-1pt)}},
      dash pattern=on 3pt off 3pt,
      line width=1pt,
      draw=color2
      },
    preaction={
      transform canvas={shift={(0pt,-2.5pt)}},
      dash pattern=on 3pt off 3pt,
      line width=1pt,
      draw=color6
      }  
    },
    ntkdntkblackcolor1color2color6/.style={
    transform canvas={shift={(0pt,1pt)}},
    dash pattern=on 3pt off 3pt,
    line width=1pt,
    draw=color1,
    preaction={
      transform canvas={shift={(0pt,2.5pt)}},
      line width=1pt,
      draw=black
      },
    preaction={
      transform canvas={shift={(0pt,-1pt)}},
      dash pattern=on 3pt off 3pt,
      line width=1pt,
      draw=color2
      },
    preaction={
      transform canvas={shift={(0pt,-2.5pt)}},
      dash pattern=on 3pt off 3pt,
      line width=1pt,
      draw=color6
      }  
    },
     ntkdntkcolor6color1color2/.style={
    transform canvas={shift={(0pt,2.5pt)}},
    dash pattern=on 3pt off 3pt,
    line width=1pt,
    draw=color6,
    preaction={
      transform canvas={shift={(0pt,1pt)}},
      dash pattern=on 3pt off 3pt,
      line width=1pt,
      draw=color1
      },
    preaction={
      transform canvas={shift={(0pt,-1pt)}},
      dash pattern=on 3pt off 3pt,
      line width=1pt,
      draw=color2
      }  
    },
    ntkdntkcolor6color1color2black/.style={
    transform canvas={shift={(0pt,2.5pt)}},
    dash pattern=on 3pt off 3pt,
    line width=1pt,
    draw=color6,
    preaction={
      transform canvas={shift={(0pt,1pt)}},
      dash pattern=on 3pt off 3pt,
      line width=1pt,
      draw=color1
      },
    preaction={
      transform canvas={shift={(0pt,-1pt)}},
      dash pattern=on 3pt off 3pt,
      line width=1pt,
      draw=color2
      },
    preaction={
      transform canvas={shift={(0pt,-2.5pt)}},
      line width=1pt,
      draw=black
      }
    }
}

%%% Local Variables:
%%% mode: LaTeX
%%% TeX-master: "ntk_feynman"
%%% End:

